A SEIR model with time-varying coefficients for analysing the SARS-CoV-2 epidemic

In this study, we propose a time-dependent Susceptible-Exposed-Infected-Recovered (SEIR) model for the analysis of the SARS-CoV-2 epidemic outbreak in three different countries, the United States of America, Italy and Iceland using public data inherent the numbers of the epidemic wave. Since several types and grades of actions were adopted by the governments, including travel restrictions, social distancing, or limitation of movement, we want to investigate how these measures can affect the epidemic curve of the infectious population. The parameters of interest for the SEIR model were estimated employing a composite likelihood approach. Moreover, standard errors have been corrected for temporal dependence. The adoption of restrictive measures results in flatten epidemic curves, and the future evolution indicated a decrease in the number of cases.

==> mybib.tex <==
% Encoding: UTF-8
@article{Chandler:Bate:2007,
	author = {Chandler, Richard E. and Bate, Steven},
	title = "{Inference for clustered data using the independence loglikelihood}",
	journal = {Biometrika},
	volume = {94},
	number = {1},
	pages = {167-183},
	year = {2007}
}
@article{Lyu:2020,
	title={Community Use Of Face Masks And {COVID-19}: Evidence From A Natural Experiment Of State Mandates In The {US}: Study examines impact on {COVID-19} growth rates associated with state government mandates requiring face mask use in public.},
	author={Lyu, Wei and Wehby, George L},
	journal={Health affairs},
	volume={39},
	number={8},
	pages={1419-1425},
	year={2020}
}
@article{Lancet:2020,
	title={{COVID-19}: too little, too late?},
	author={Lancet, The},
	journal={Lancet (London, England)},
	volume={395},
	number={10226},
	pages={755},
	year={2020},
	publisher={Elsevier}
}
@article{Godio:2020,
	title={{SEIR} modeling of the Italian epidemic of {SARS-CoV-2} using computational swarm intelligence},
	author={Godio, Alberto and Pace, Francesca and Vergnano, Andrea},
	journal={International Journal of Environmental Research and Public Health},
	volume={17},
	number={10},
	pages={3535},
	year={2020},
	publisher={Multidisciplinary Digital Publishing Institute}
}
@article{Lekone:Finkenstadt,
	author = {Lekone, Phenyo E. and Finkenst\"{a}dt, B.F.},
	title = {Statistical Inference in a Stochastic Epidemic {SEIR} Model with Control Intervention: {E}bola as a Case Study},
	journal = {Biometrics},
	volume = {62},
	number = {4},
	pages = {1170-1177},
	year = {2006}
}

@incollection{allen:2008,
	title={An introduction to stochastic epidemic models},
	author={Allen, Linda JS},
	booktitle = {Mathematical Epidemiology},
	editor={Brauer, Fred and Wu, Jianhong},
	pages =  {81-130},
	year = {2008},
	publisher={Springer},
	address={New York}
}

@book{andersson2012stochastic,
	title={Stochastic Epidemic Models and their Statistical Analysis},
	author={Andersson, Hakan and Britton, Tom},
	year={2012},
	publisher={Springer},
	address={New York}
}


@article{Dureau:2013,
	author = {Dureau, Joseph and Kalogeropoulos, Konstantinos and Baguelin, Marc},
	title = "{Capturing the time-varying drivers of an epidemic using stochastic dynamical systems}",
	journal = {Biostatistics},
	volume = {14},
	number = {3},
	pages = {541-555},
	year = {2013},
}


@article {Ionides:2006,
	author = {Ionides, E. L. and Bret{\'o}, C. and King, A. A.},
	title = {Inference for nonlinear dynamical systems},
	volume = {103},
	number = {49},
	pages = {18438--18443},
	year = {2006},
	publisher = {National Academy of Sciences},
	journal = {Proceedings of the National Academy of Sciences}
}

@article{Finkesdadt:Grenfell:2000,
	author = {Finkenst\"{a}dt, B. F. and Grenfell, B. T.},
	title = {Time series modelling of childhood diseases: a dynamical systems approach},
	journal = {Journal of the Royal Statistical Society: Series C (Applied Statistics)},
	volume = {49},
	number = {2},
	pages = {187-205},
	year = {2000}
}

@article{Jacod:Sorensen:2018,
	author = {Jacod, Jean and - S\o{}rensen, Michael},
	title = {A review of asymptotic theory of estimating functions},
	journal = {Statistical Inference for Stochastic Processes},
	year = {2018},
	volume = {21},
		number = {2},
	pages = {415-434}
}

@article{anderson2020will,
	title={How will country-based mitigation measures influence the course of the {COVID-19} epidemic?},
	author={Anderson, Roy M and Heesterbeek, Hans and Klinkenberg, Don and Hollingsworth, T D{\'e}irdre},
	journal={The Lancet},
	volume={395},
	number={10228},
	pages={931--934},
	year={2020}
}
@article{Andrews:1991,
	author = {Donald W. K. Andrews},
	journal = {Econometrica},
	 title = {Heteroskedasticity and autocorrelation consistent covariance matrix estimation},
	pages = {817--858},
	volume = {59},
		number={3},
	year = {1991}
}

@article{Lindsay:1988,
	author = {Lindsay, B.G.},
	title = {Composite likelihood methods},
	journal = {Contemporary Mathematics},
	year = {1988},
	volume = {80},
		number={1},
	pages = {221-239}
}


@InCollection{Hindmarsh:1983,
  author    = {Hindmarsh, A.C.},
  booktitle = {Scientific Computing},
  title     = {ODEPACK, A Systematized Collection of ODE Solvers},
  editor    = {Stepleman, R. S.},
  pages     = {55-64},
  publisher = {North-Holland},
  address ={Amsterdam},
  year      = {1983},
}



@book{anderson1992,
	title={Infectious diseases of humans: dynamics and control},
	author={Anderson, Roy M and Anderson, B and May, Robert M},
	year={1992},
	publisher={Oxford University Press},
	address={Oxford}
}
@article{boatto2018,
	title={{SIR} model with time dependent infectivity parameter: approximating the epidemic attractor and the importance of the initial phase},
	author={Boatto, Stefanella and Bonnet, Catherine and Cazelles, Bernard and Mazenc, Fr{\'e}d{\'e}ric},
	journal={open archive HAL},
	volume = {hal-01677886},
	year={2018}
}

@article{boily2007,
	title={Evaluating large-scale {HIV} prevention interventions: study design for an integrated mathematical modelling approach},
	author={Boily, Marie-Claude and Lowndes, CM and Vickerman, Peter and Kumaranayake, Lilani and Blanchard, James and Moses, Stephen and Ramesh, BM and Pickles, Michael and Watts, Charlotte and Washington, Reynold and others},
	journal={Sexually Transmitted Infections},
	volume={83},
	number={7},
	pages={582--589},
	year={2007},
	publisher={The Medical Society for the Study of Venereal Disease}
}
@article{chavez2017,
	title={A {SIR-D}engue transmission model with seasonal effects and impulsive control},
	author={Ch{\'a}vez, Joseph P{\'a}ez and G{\"o}tz, Thomas and Siegmund, Stefan and Wijaya, Karunia Putra},
	journal={Mathematical Biosciences},
	volume={289},
	number={1},
	pages={29--39},
	year={2017},
	publisher={Elsevier}
}
@article{chowell2017fitting,
	title={Fitting dynamic models to epidemic outbreaks with quantified uncertainty: a primer for parameter uncertainty, identifiability, and forecasts},
	author={Chowell, Gerardo},
	journal={Infectious Disease Modelling},
	volume={2},
	number={3},
	pages={379--398},
	year={2017},
	publisher={Elsevier}
}
@misc{csse2020,
	title={Coronavirus {COVID-19} Global Cases by the {Center for Systems Science and Engineering (CSSE) at Johns Hopkins University} ({JHU})},
	author={CSSE, JHU},
	year={2020}
}
@article{currie2004,
	title={Smoothing and forecasting mortality rates},
	author={Currie, Iain D and Durban, Maria and Eilers, Paul HC},
	journal={Statistical Modelling},
	volume={4},
	number={4},
	pages={279--298},
	year={2004},
	publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}
@article{dong2020,
	title={An interactive web-based dashboard to track {COVID-19} in real time},
	author={Dong, Ensheng and Du, Hongru and Gardner, Lauren},
	journal={The Lancet infectious diseases},
	volume={20},
	number={5},
	pages={533--534},
	year={2020},
	publisher={Elsevier}
}

@book{efron1994,
	title={An introduction to the bootstrap},
	author={Efron, Bradley and Tibshirani, Robert J},
	year={1994},
	publisher={CRC press}
}
@article{eilers1996,
	title={Flexible smoothing with B-splines and penalties},
	author={Eilers, Paul HC and Marx, Brian D},
	journal={Statistical science},
	pages={89--102},
	year={1996},
	publisher={JSTOR}
}
@article{eurosurveillance2020,
	title={Note from the editors: {World Health Organization} declares novel coronavirus ({2019-nCoV}) sixth public health emergency of international concern},
	author={Eurosurveillance Editorial Team and others},
	journal={Eurosurveillance},
	volume={25},
	number={5},
	pages={200131e},
	year={2020},
	publisher={European Centre for Disease Prevention and Control}
}

@article{fang2020,
year = {2020},
 publisher = {Wiley},
  volume = {92},
  number = {6},
  pages = {645--659},
  author = {Yaqing Fang and Yiting Nie and Marshare Penny},
  title = {Transmission dynamics of the {COVID}-19 outbreak and effectiveness of government interventions: A data-driven analysis},
  journal = {Journal of Medical Virology}
}
@techreport{ferguson2020,
author = {Ferguson, Neil and Laydon, Daniel and Nedjati Gilani, Gemma and Imai, Natsuko and Ainslie, Kylie and Baguelin, Marc and Bhatia, Sangeeta and Boonyasiri, Adhiratha and Cucunuba Perez, ZULMA and Cuomo-Dannenburg, Gina and others},
  institution = {Imperial College London},
  title       = {Report 9: Impact of non-pharmaceutical interventions (NPIs) to reduce {COVID-19} mortality and healthcare demand},
  year        = {2020}
}

@article{flaxman2020,
	title={Report 13: Estimating the number of infections and the impact of non-pharmaceutical interventions on {COVID-19} in 11 {E}uropean countries},
	author={Flaxman, Seth and Mishra, Swapnil and Gandy, Axel and Unwin, H and Coupland, H and Mellan, T and Zhu, H and Berah, T and Eaton, J and Perez Guzman, P and others},
	  journal={arXiv e-prints},
	year={2020}
}
@article{gudbjartsson2020,
	title={Spread of {SARS-CoV-2} in the Icelandic population},
	author={Gudbjartsson, Daniel F and Helgason, Agnar and Jonsson, Hakon and Magnusson, Olafur T and Melsted, Pall and Norddahl, Gudmundur L and Saemundsdottir, Jona and Sigurdsson, Asgeir and Sulem, Patrick and Agustsdottir, Arna B and others},
	journal={New England Journal of Medicine},
	volume={382},
	number={24},
	pages={2302--2315},
	year={2020},
	publisher={Mass Medical Soc}
}
@article{haas2020,
	title={Coronavirus and risk analysis},
	year = {2020},
	volume = {40},
	number = {4},
	pages = {660--661},
	author = {Charles Haas},
	journal = {Risk Analysis}
}

@article{hong2020,
	title={Estimation of time-varying reproduction numbers underlying epidemiological processes: A new statistical tool for the {COVID-19} pandemic},
	author={Hong, Hyokyoung G and Li, Yi},
	journal={PloS one},
	volume={15},
	number={7},
	pages={e0236464},
	year={2020},
	publisher={Public Library of Science San Francisco, CA USA}
}


@article{hooker2011,
	title={Parameterizing state--space models for infectious disease dynamics by generalized profiling: measles in {O}ntario},
	author={Hooker, Giles and Ellner, Stephen P and Roditi, Laura De Vargas and Earn, David JD},
	journal={Journal of the Royal Society Interface},
	volume={8},
	number={60},
	pages={961--974},
	year={2011},
	publisher={The Royal Society}
}

@article{kermack1927,
	title={A contribution to the mathematical theory of epidemics},
	author={Kermack, William Ogilvy and McKendrick, Anderson G},
	journal={Proceedings of the Royal Society of London, Series A},
	volume={115},
	number={772},
	pages={700--721},
	year={1927},
	publisher={The Royal Society London}
}


@article{kucharski2020,
	title={Early dynamics of transmission and control of {COVID-19}: a mathematical modelling study},
	author={Kucharski, Adam J and Russell, Timothy W and Diamond, Charlie and Liu, Yang and Edmunds, John and Funk, Sebastian and Eggo, Rosalind M and Sun, Fiona and Jit, Mark and Munday, James D and others},
	journal={The Lancet Infectious Diseases},
volume={20},
number={5},
pages={553--558},
year={2020},
publisher={Elsevier}
}
@article{lavezzo2020,
	title={Suppression of a {SARS-CoV-2} outbreak in the Italian municipality of {Vo’}},
	author={Lavezzo, Enrico and Franchin, Elisa and Ciavarella, Constanze and Cuomo-Dannenburg, Gina and Barzon, Luisa and Del Vecchio, Claudia and Rossi, Lucia and Manganelli, Riccardo and Loregian, Arianna and Navarin, Nicol{\`o} and others},
	journal={Nature},
	volume={584},
	number={7821},
	pages={425--429},
	year={2020},
	publisher={Nature Publishing Group}
}
@article{liu2012,
	title={Infectious disease models with time-varying parameters and general nonlinear incidence rate},
	author={Liu, Xinzhi and Stechlinski, Peter},
	journal={Applied Mathematical Modelling},
	volume={36},
	number={5},
	pages={1974--1994},
	year={2012},
	publisher={Elsevier}
}
@article{liu2020,
	title={The reproductive number of {COVID-19} is higher compared to {SARS} coronavirus},
	author={Liu, Ying and Gayle, Albert A and Wilder-Smith, Annelies and Rockl{\"o}v, Joacim},
	journal={Journal of Travel Medicine},
	year={2020}
}
@article{morettini2020,
	title={{COVID-19} in {I}taly: Dataset of the {I}talian {C}ivil {P}rotection {D}epartment},
	author={Morettini, Micaela and Sbrollini, Agnese and Marcantoni, Ilaria and Burattini, Laura},
	journal={Data in Brief},
	pages={105526},
	year={2020},
	publisher={Elsevier}
}

@article{parodi2020,
	title={From containment to mitigation of {COVID-19} in the {US}},
	author={Parodi, Stephen M and Liu, Vincent X},
	journal={Journal of American Medical Association},
	year={2020},
	pages={1441},
	volume={323}, 
	DOI={10.1001/jama.2020.3882}, 
	number={15}
}

@article{parmet2020,
	title={{COVID-19} -- the law and limits of quarantine},
	author={Parmet, Wendy E and Sinha, Michael S},
	journal={New England Journal of Medicine},
	volume={382},
	number={15},
	pages={e28},
	year={2020},
	publisher={Mass Medical Soc}
}

@article{peng2020,
	title={Epidemic analysis of {COVID-19} in {C}hina by dynamical modeling},
	author={Peng, Liangrong and Yang, Wuyue and Zhang, Dongyan and Zhuge, Changjing and Hong, Liu},
	journal={arXiv preprint arXiv:2002.06563},
	year={2020}
}

@article{petropoulos2020,
	title={Forecasting the novel coronavirus {COVID-19}},
	author={Petropoulos, Fotios and Makridakis, Spyros},
	journal={PLOS One},
	volume={15},
	number={3},
	pages={e0231236},
	year={2020},
	publisher={Public Library of Science San Francisco, CA USA}
}
@article{piccolomini2020,
title={Monitoring Italian {COVID-19} spread by a forced {SEIRD} model},
author={Loli Piccolomini, Elena and Zama, Fabiana},
journal={PloS one},
volume={15},
number={8},
pages={e0237417},
year={2020},
publisher={Public Library of Science San Francisco, CA USA}
}

@Manual{R2019,
    title = {R: {A} Language and {E}nvironment for {S}tatistical {C}omputing},
    author = {{R Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2019}
  }
@article{remuzzi2020,
	title={{COVID-19} and {I}taly: what next?},
	year = {2020},
	volume = {395},
	number = {10231},
	pages = {1225--1228},
	author={Remuzzi, Andrea and Remuzzi, Giuseppe},
	journal={The Lancet},
	publisher={Elsevier}
}
@article{rubino2020,
	title={As {COVID-19} cases, deaths and fatality rates surge in {I}taly, underlying causes require investigation},
	author={Rubino, Salvatore and Kelvin, Nikki and Bermejo-Martin, Jes{\'u}s F and Kelvin, David},
	journal={The Journal of Infection in Developing Countries},
	volume={14},
	number={3},
	pages={265--267},
	year={2020}
}
@article{smirnova2019forecasting,
	title={Forecasting epidemics through nonparametric estimation of time-dependent transmission rates using the {SEIR} model},
	author={Smirnova, Alexandra and deCamp, Linda and Chowell, Gerardo},
	journal={Bulletin of mathematical biology},
	volume={81},
	number={11},
	pages={4343--4365},
	year={2019},
	publisher={Springer}
}
@article{stock2020,
	title={Estimates of the undetected rate among the {SARS-COV-2} infected using testing data from {I}celand},
	author={Stock, James H and Aspelund, Karl M and Droste, Michael and Walker, Christopher D},
	journal={medRxiv},
	year={2020},
	publisher={Cold Spring Harbor Laboratory Press}
}
@article{unkel2012,
	title={Statistical methods for the prospective detection of infectious disease outbreaks: a review},
	author={Unkel, Steffen and Farrington, C Paddy and Garthwaite, Paul H and Robertson, Chris and Andrews, Nick},
	journal={Journal of the Royal Statistical Society: Series A (Statistics in Society)},
	volume={175},
	number={1},
	pages={49--82},
	year={2012},
	publisher={Wiley Online Library}
}
@article{varin2005,
	title={A note on composite likelihood inference and model selection},
	author={Varin, Cristiano and Vidoni, Paolo},
	journal={Biometrika},
	volume={92},
	number={3},
	pages={519--528},
	year={2005},
	publisher={Oxford University Press}
}
@article{wang1995,
	title={Bootstrap confidence intervals for smoothing splines and their comparison to Bayesian confidence intervals},
	author={Wang, Yuedong and Wahba, Grace},
	journal={Journal of Statistical Computation and Simulation},
	volume={51},
	number={2-4},
	pages={263--279},
	year={1995},
	publisher={Taylor \& Francis}
}
@article{wang2020,
	title={Phase-adjusted estimation of the number of coronavirus disease 2019 cases in {W}uhan, {C}hina},
	author={Wang, Huwen and Wang, Zezhou and Dong, Yinqiao and Chang, Ruijie and Xu, Chen and Yu, Xiaoyue and Zhang, Shuxian and Tsamlag, Lhakpa and Shang, Meili and Huang, Jinyan and others},
	journal={Cell Discovery},
	volume={6},
	number={1},
	pages={1--8},
	year={2020},
	publisher={Nature Publishing Group}
}

@techreport{who2020,
	title={Coronavirus disease 2019 ({COVID-19}): situation report, 72},
	author={{World Health Organization} and others},
	year={2020},
	publisher={World Health Organization}
}

@article{wu2020,
	title={Nowcasting and forecasting the potential domestic and international spread of the {2019-nCoV} outbreak originating in {W}uhan, {C}hina: a modelling study},
	author={Wu, Joseph T and Leung, Kathy and Leung, Gabriel M},
	journal={The Lancet},
	volume={395},
	number={10225},
	pages={689--697},
	year={2020},
	publisher={Elsevier}
}

@article{zhang2020,
	title={Prediction of the {COVID-19} outbreak based on a realistic stochastic model},
	author={Zhang, Yuan and You, Chong and Cai, Zhenghao and Sun, Jiarui and Hu, Wenjie and Zhou, Xiao-Hua},
	journal={medRxiv},
	year={2020},
	publisher={Cold Spring Harbor Laboratory Press}
}

@Comment{jabref-meta: databaseType:biblatex;}

